A Nonparametric Bayes Approach to Online Activity Prediction

Accurately predicting the onset of specific activities within defined timeframes holds significant importance in several applied contexts. In particular, accurate prediction of the number of future users that will be exposed to an intervention is an important piece of information for experimenters running online experiments (A/B tests). In this work, we propose a novel approach to predict the number of users that will be active in a given time period, as well as the temporal trajectory needed to attain a desired user participation threshold. We model user activity using a Bayesian nonparametric approach which allows us to capture the underlying heterogeneity in user engagement. We derive closed-form expressions for the number of new users expected in a given period, and a simple Monte Carlo algorithm targeting the posterior distribution of the number of days needed to attain a desired number of users; the latter is important for experimental planning. We illustrate the performance of our approach via several experiments on synthetic and real world data, in which we show that our novel method outperforms existing competitors.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> shortcuts.tex <==
% \usepackage{arxiv}
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{amsmath, amssymb}
\usepackage{hyperref}

\usepackage{bm}
\usepackage{graphicx}
\usepackage{sidecap}
\usepackage[toc,page]{appendix}
\usepackage{float}
\usepackage{amsthm}
\usepackage{bbm}
\usepackage{cancel}
\usepackage{multirow}
\usepackage{natbib}
\usepackage[table,xcdraw]{xcolor}
\usepackage{cleveref}

\def\vATE{\bm{\mathrm{ATE}}}

\def\ATE{\mathrm{ATE}}
\def\gATE{\mathrm{gATE}}

\def\unATE{\widehat{\ATE}_{\text{unadj}}}
\def\vunATE{\widehat{\bm{\ATE}}_{\text{unadj}}}

\def\adjATE{\widehat{\ATE}_{\text{adj}}}
\def\adjATEf{\widehat{\ATE}_{\text{adj},0}}
\def\intATE{\widehat{\ATE}_{\text{interact}}}

\def\ungATE{\widehat{\gATE}_{\text{unadj}}}
\def\adjgATE{\widehat{\gATE}_{\text{adj}}}
\def\intgATE{\widehat{\gATE}_{\text{interact}}}

\def\unSigma{\widehat{\bm{\Sigma}}_{\text{unadj}}}
\def\adjSigma{\widehat{\bm{\Sigma}}_{\text{adj}}}
\def\intSigma{\widehat{\bm{\Sigma}}_{\text{interact}}}
\def\adjtheta{\hat{\bm{\theta}}_{\text{adj}}}
\def\inttheta{\hat{\bm{\theta}}_{\text{interact}}}
\def\adjh{h_{\text{adj}}}
\def\inth{h_{\text{interact}}}
\def\adjf{f_{\text{adj}}}
\def\intf{f_{\text{interact}}}
\def\intSigma{\bm{\Sigma}_{\text{interact}}}
\def\adjSigma{\bm{\Sigma}_{\text{adj}}}
\def\intGamma{\bm{\Gamma}_{\text{interact}}}
\def\adjGamma{\bm{\Gamma}_{\text{adj}}}
\def\intgATE{\widehat{\mathrm{gATE}}_{\text{interact}}}
\def\hatATE{\widehat{\mathrm{ATE}}}
\def\hatgATE{\widehat{\mathrm{gATE}}}

\def\sigmasqungATE{\sigma^2_{\text{gATE}_{\text{unadj}}}}
\def\de{\mathrm{d}}
\def\EE{\mathbb{E}}
\def\XX{\mathbb{X}}
\def\PP{\mathbb{P}}
\def\WW{\mathbb{W}}
\def\RE{\mathbb{R}}
\def\VV{\mathcal{V}}
\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}
\def\HH{\mathcal{H}}
\def\ZED{\mathcal{Z}}
\def\R{\mathbb{R}}
\def\indicator{\mathbbm{1}}
\def\gibbsp{\psi}
\def\NGGP{\mathrm{NGGP}}
\def\Bern{\Bernoulli}
\def\Laplace{\mathrm{Laplace}}
\def\Dir{\mathrm{Dir}}
\def\NIG{\mathrm{NIG}}
\def\CM{\mathrm{CM}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ST}{\mathcal{S}}
\newcommand{\PPC}{\mathcal{P}^{\text{canon}}}
\newcommand{\PML}{p_{\ML}^{(\hat{y}, B, \lambda)}}
\newcommand{\tG}{\tilde{\Gamma}}
\newcommand{\LSE}{\mathrm{LSE}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\AVar}{\mathrm{AVar}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\ACov}{\mathrm{ACov}}
\newcommand{\ii}{\mathfrak{i}}
\newcommand{\iist}{\mathfrak{i}^*}
\newcommand{\jj}{\mathfrak{j}}
\newcommand{\jjst}{\mathfrak{j}^*}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\spi}{\mathrm{spill}}
\newcommand{\pa}{\mathrm{pairs}}
\newcommand{\yf}{\hat{\bar{y}}_{\text{f}}}
\newcommand{\adjbeta}{\bm{\hat{\beta}_{\text{adj}}}}
\newcommand{\adjbetaA}{\hat{\beta}_{\text{adj}, A}}
\newcommand{\adjbetaB}{\hat{\beta}_{\text{adj}, B}}
\newcommand{\intbeta}{\bm{\hat{\beta}_{\text{interact}}}}
\newcommand{\intbetaA}{\hat{\beta}_{\text{interact}, A}}
\newcommand{\intbetaB}{\hat{\beta}_{\text{interact}, B}}
\newcommand{\zi}{\bm{z}_i}
\newcommand{\zbar}{\bar{\bm{z}}}
\newcommand{\zbarA}{\bar{\bm{z}}_A}
\newcommand{\zbarB}{\bar{\bm{z}}_B}
\newcommand{\prob}{{\mathsf P}}
\newcommand{\iid}{\stackrel{\mbox{\scriptsize iid}}{\sim}}
\newcommand{\ind}{\stackrel{\mbox{\scriptsize ind}}{\sim}}



\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\newtheorem{condition}[theorem]{Condition}


